New Sufficient Conditions for Multiple-Access Channel with Correlated Sources

The problem of three-user Multiple-Access Channel (MAC) with correlated sources is investigated. An extension to the Cover-El Gamal-Salehi (CES) scheme is introduced. We use a combination of this scheme with linear codes and propose a new coding strategy. We derive new sufficient conditions to transmit correlated sources reliably. We consider an example of three-user MAC with binary inputs. Using this example, we show strict improvements over the CES scheme.

==> MAC_Correlated_Sources_Intro.tex <==
The separation principle of Shannon plays a fundamental role to reinforces the notion of modularity  which yields separate development in designing source and channel codes for communication systems. However, the separation does not generalize to multi-terminal communications as Shannon first showed it in \cite{Shannon}.

This phenomena was also observed in many-to-one communications involving transmission of correlated sources over Multiple-Access Channel (MAC), \cite{CES}. In this setup, there are multiple transmitters, each observing a source correlated to others. The transmitters do not communicate with each other and are wishing to send their observations via a MAC to a central receiver. The receiver wants to reproduce the sources with no loss.

The separate source-channel coding approach for this problem investigated in two directions.
%There are two different approaches to this problem. In the first approach the sources first compressed using a source coding scheme then a channle code is used to send the outputs of the source-encoders to via the MAC. In the other approach, a joint source-channel code is designed to map the source sequences directly to the channel's inputs. For the first case, there are two directions in the literature.  
In one direction (channel coding), Ahlswede \cite{Ahlswede-MAC} and Liao \cite{Liao} studied the case where the transmitters have independent information and derived the capacity region for channel coding over MAC. In another direction, the distributed source coding problem was studied in which transmitters can communicate to the receiver error-free.  Slepian and Wolf  showed that lossless reproduction of the sources is possible with rates close to the joint entropy, \cite{Slepian-Wolf_dist}.


Due to suboptimality of the separation based strategies, the joint-source coding approach has been of great interests, \cite{Gunduz-Goldsmith}. The authors of \cite{CES} introduced the Cover-El Gamal-Salehi (CES) scheme and generalized the results of \cite{Ahlswede-MAC} and \cite{Slepian-Wolf_MAC}. They also gave a single-letter characterization of the set of sources that can be reliably transmitted and showed that this scheme strictly improves upon the previously known schemes. However, Dueck \cite{Dueck} showed that this approach gives only a sufficient condition and not a necessary one. The joint source-channel coding approach is not limited to this problem and is well studied in other settings such as: source coding with side information via a MAC \cite{Ahlswede-MAC-With-Side-info}, broadcast channels with correlated sources \cite{Han-Costa-BC} and interference channels \cite{Salehi-Kurtas-IS}.

Recently, structured codes are used to design coding strategies for joint source-channel coding problems, \cite{Pradhan-Choi, Choi-Pradhan, Nazer_Gasper_Comp_MAC, Arun_comp_over_MAC_ISIT13, transversal}. A a graph-theoretic framework was introduced in  \cite{Pradhan-Choi, Choi-Pradhan} to improve the source-channel coding scheme both in MAC and broacast channel. 


In this work, we study the three-user version of MAC with correlated sources. We first extend the CES scheme to this problem and derive an achievable rate region. As shown is in \cite{CES}, this coding strategy improves upon separate source-channel coding techniques by choosing the codewords that are statistically depended on the distribution of the sources. We observe that further improvements are possible when the sources impose an algebraic structure. For example when one of the sources is the modulo sum of the other two. In this scenario, an structure coding strategy is needed to match better with the structure of the sources. With this intuition, we use a combination of linear codes and the CES scheme to derive a new achievable region. Through an example, we show strict improvements over the CES scheme.

The rest of this paper is as follows: In section \ref{sec: priliminaries}, we provide the notations, definitions and the problem statement. In Section \ref{sec: CES_extension} an extension of the CES scheme for three-user MAC with correlated sources is discussed. A new coding scheme based on linear codes is provided in Section \ref{sec: proposed scheme} and the improvements over the CES scheme is discussed in Section \ref{sec: improvements over CES}. Lastly Section \ref{sec: conclusion} concludes the paper. 
\section{Priliminaries and Problem Statement}\label{sec: priliminaries}

